Learning Multiple Sound Source 2D Localization

In this paper, we propose novel deep learning based algorithms for multiple sound source localization. Specifically, we aim to find the 2D Cartesian coordinates of multiple sound sources in an enclosed environment by using multiple microphone arrays. To this end, we use an encoding-decoding architecture and propose two improvements on it to accomplish the task. In addition, we also propose two novel localization representations which increase the accuracy. Lastly, new metrics are developed relying on resolution-based multiple source association which enables us to evaluate and compare different localization approaches. We tested our method on both synthetic and real world data. The results show that our method improves upon the previous baseline approach for this problem.

==> tables/resarcsynth.tex <==
\begin{table*}[bt]
\footnotesize\addtolength{\tabcolsep}{-5pt}
\begin{center}
\begin{tabular}{|c|
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{EFEFEF}}c cc|
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{EFEFEF}}c cc|
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{EFEFEF}}c cc|
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{EFEFEF}}c cc|
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{EFEFEF}}c cc|
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{EFEFEF}}c cc|}
\hline
\cellcolor[HTML]{FFFFFF}Resolution          & \multicolumn{12}{c|}{\cellcolor[HTML]{FFFFFF}0.3 m}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                           & \multicolumn{12}{c|}{\cellcolor[HTML]{FFFFFF}1 m}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                           \\ \hline
\cellcolor[HTML]{FFFFFF}Sources             & \multicolumn{4}{c|}{\cellcolor[HTML]{FFFFFF}1}                                                                                                                                                & \multicolumn{4}{c|}{\cellcolor[HTML]{FFFFFF}2}                                                                                                                                                & \multicolumn{4}{c|}{\cellcolor[HTML]{FFFFFF}Overall}                                                                                                                                          & \multicolumn{4}{c|}{\cellcolor[HTML]{FFFFFF}1}                                                                                                                                                                                              & \multicolumn{4}{c|}{\cellcolor[HTML]{FFFFFF}2}                                                                                                                                                & \multicolumn{4}{c|}{\cellcolor[HTML]{FFFFFF}Overall}                                                                                                                                          \\ \hline
\cellcolor[HTML]{FFFFFF}Metrics             & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Pre} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Rec} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}F1} & \cellcolor[HTML]{FFFFFF}RMSE          & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Pre} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Rec} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}F1} & \cellcolor[HTML]{FFFFFF}RMSE          & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Pre} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Rec} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}F1} & \cellcolor[HTML]{FFFFFF}RMSE          & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}{\color[HTML]{000000} Pre}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}{\color[HTML]{000000} Rec}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}F1} & \cellcolor[HTML]{FFFFFF}RMSE          & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Pre} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Rec} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}F1} & \cellcolor[HTML]{FFFFFF}RMSE          & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Pre} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Rec} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}F1} & \cellcolor[HTML]{FFFFFF}RMSE          \\ \hline
\cellcolor[HTML]{FFFFFF}Mono-encoder        & \textbf{1.00}                                    & \textbf{1.00}                                    & \cellcolor[HTML]{FFFFFF}\textbf{1.00}           & \cellcolor[HTML]{FFFFFF}\textbf{0.05} & 0.88                                             & 0.81                                             & \cellcolor[HTML]{FFFFFF}0.84                    & \cellcolor[HTML]{FFFFFF}0.12          & 0.92                                             & 0.87                                             & \cellcolor[HTML]{FFFFFF}0.90                    & \cellcolor[HTML]{FFFFFF}0.10          & {\color[HTML]{000000} \textbf{1.00}}                                    & {\color[HTML]{000000} \textbf{1.00}}                                    & \cellcolor[HTML]{FFFFFF}\textbf{1.00}           & \cellcolor[HTML]{FFFFFF}0.06          & 0.98                                             & 0.90                                             & \cellcolor[HTML]{FFFFFF}0.94                    & \cellcolor[HTML]{FFFFFF}0.19          & \textbf{0.99}                                    & 0.93                                             & \cellcolor[HTML]{FFFFFF}0.96                    & \cellcolor[HTML]{FFFFFF}0.16          \\
\cellcolor[HTML]{FFFFFF}Multi-encoder       & \textbf{1.00}                                    & \textbf{1.00}                                    & \cellcolor[HTML]{FFFFFF}\textbf{1.00}           & \cellcolor[HTML]{FFFFFF}\textbf{0.05} & 0.91                                             & 0.82                                             & \cellcolor[HTML]{FFFFFF}0.86                    & \cellcolor[HTML]{FFFFFF}\textbf{0.09} & 0.94                                             & 0.88                                             & \cellcolor[HTML]{FFFFFF}0.91                    & \cellcolor[HTML]{FFFFFF}\textbf{0.09} & {\color[HTML]{000000} \textbf{1.00}}                                    & {\color[HTML]{000000} \textbf{1.00}}                                    & \cellcolor[HTML]{FFFFFF}\textbf{1.00}           & \cellcolor[HTML]{FFFFFF}\textbf{0.05} & 0.98                                             & 0.89                                             & \cellcolor[HTML]{FFFFFF}0.93                    & \cellcolor[HTML]{FFFFFF}0.18          & \textbf{0.99}                                    & 0.93                                             & \cellcolor[HTML]{FFFFFF}0.96                    & \cellcolor[HTML]{FFFFFF}0.14          \\
\cellcolor[HTML]{FFFFFF}Full                & \textbf{1.00}                                    & \textbf{1.00}                                    & \cellcolor[HTML]{FFFFFF}\textbf{1.00}           & \cellcolor[HTML]{FFFFFF}0.06          & \textbf{0.93}                                    & \textbf{0.86}                                    & \cellcolor[HTML]{FFFFFF}\textbf{0.89}           & \cellcolor[HTML]{FFFFFF}0.10          & \textbf{0.95}                                    & \textbf{0.91}                                    & \cellcolor[HTML]{FFFFFF}\textbf{0.93}           & \cellcolor[HTML]{FFFFFF}\textbf{0.09} & {\color[HTML]{000000} \textbf{1.00}}                                    & {\color[HTML]{000000} \textbf{1.00}}                                    & \cellcolor[HTML]{FFFFFF}\textbf{1.00}           & \cellcolor[HTML]{FFFFFF}0.06          & \textbf{0.99}                                    & \textbf{0.92}                                    & \cellcolor[HTML]{FFFFFF}\textbf{0.95}           & \cellcolor[HTML]{FFFFFF}\textbf{0.16} & \textbf{0.99}                                    & \textbf{0.95}                                    & \cellcolor[HTML]{FFFFFF}\textbf{0.97}           & \cellcolor[HTML]{FFFFFF}\textbf{0.13} \\ \hline
\cellcolor[HTML]{FFFFFF}Mono-encoder (10\%) & 0.92                                             & 0.91                                             & \cellcolor[HTML]{FFFFFF}0.92                    & \cellcolor[HTML]{FFFFFF}0.12          & 0.74                                             & 0.45                                             & \cellcolor[HTML]{FFFFFF}0.56                    & \cellcolor[HTML]{FFFFFF}0.15          & 0.82                                             & 0.61                                             & \cellcolor[HTML]{FFFFFF}0.70                    & \cellcolor[HTML]{FFFFFF}0.14          & {\color[HTML]{000000} \textbf{1.00}}                                    & {\color[HTML]{000000} 0.99}                                             & \cellcolor[HTML]{FFFFFF}0.99                    & \cellcolor[HTML]{FFFFFF}0.17          & 0.96                                             & 0.58                                             & \cellcolor[HTML]{FFFFFF}0.73                    & \cellcolor[HTML]{FFFFFF}0.28          & \textbf{0.98}                                    & 0.72                                             & \cellcolor[HTML]{FFFFFF}0.83                    & \cellcolor[HTML]{FFFFFF}0.23          \\
Multi-encoder (10\%)                        & 0.98                                             & 0.98                                             & 0.98                                            & \textbf{0.09}                         & \textbf{0.84}                                    & 0.56                                             & 0.67                                            & 0.14                                  & \textbf{0.90}                                    & 0.70                                             & 0.79                                            & 0.12                                  & \textbf{1.00}                                                           & \textbf{1.00}                                                           & \textbf{1.00}                                   & 0.11                                  & \textbf{0.97}                                    & 0.65                                             & 0.78                                            & \textbf{0.22}                         & \textbf{0.98}                                    & 0.77                                             & 0.86                                            & \textbf{0.18}                         \\
Full (10\%)                                 & \textbf{0.99}                                    & \textbf{0.99}                                    & \textbf{0.99}                                   & \textbf{0.09}                         & \textbf{0.84}                                    & \textbf{0.60}                                    & \textbf{0.70}                                   & \textbf{0.13}                         & \textbf{0.90}                                    & \textbf{0.73}                                    & \textbf{0.81}                                   & \textbf{0.11}                         & \textbf{1.00}                                                           & \textbf{1.00}                                                           & \textbf{1.00}                                   & \textbf{0.10}                         & \textbf{0.97}                                    & \textbf{0.69}                                    & \textbf{0.81}                                   & \textbf{0.22}                         & \textbf{0.98}                                    & \textbf{0.80}                                    & \textbf{0.88}                                   & \textbf{0.18}                         \\ \hline
\end{tabular}
\end{center}
\normalsize
\caption{Architecture results on synthetic test set}
\label{tab:resarcsynth}
\end{table*}




==> tables/resrepreal.tex <==
\begin{table*}[bt]
\footnotesize\addtolength{\tabcolsep}{-5pt}
\begin{center}
\begin{tabular}{|
>{\columncolor[HTML]{FFFFFF}}c |
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c |
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c |
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c |
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c |
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c |
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c |}
\hline
Resolution            & \multicolumn{12}{c|}{\cellcolor[HTML]{FFFFFF}0.3 m}                                                                                                                                                                                                                                                                                                                                                                                                                                                                   & \multicolumn{12}{c|}{\cellcolor[HTML]{FFFFFF}1 m}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                   \\ \hline
Sources               & \multicolumn{4}{c|}{\cellcolor[HTML]{FFFFFF}1}                                                                                                                        & \multicolumn{4}{c|}{\cellcolor[HTML]{FFFFFF}2}                                                                                                                        & \multicolumn{4}{c|}{\cellcolor[HTML]{FFFFFF}Overall}                                                                                                                  & \multicolumn{4}{c|}{\cellcolor[HTML]{FFFFFF}1}                                                                                                                                                                      & \multicolumn{4}{c|}{\cellcolor[HTML]{FFFFFF}2}                                                                                                                        & \multicolumn{4}{c|}{\cellcolor[HTML]{FFFFFF}Overall}                                                                                                                  \\ \hline
Metrics               & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Pre} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Rec} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}F1} & RMSE          & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Pre} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Rec} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}F1} & RMSE          & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Pre} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Rec} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}F1} & RMSE          & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}{\color[HTML]{000000} Pre}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}{\color[HTML]{000000} Rec}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}F1} & RMSE          & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Pre} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Rec} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}F1} & RMSE          & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Pre} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Rec} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}F1} & RMSE          \\ \hline
Tight grid (naive)    & 0.19                                             & \textbf{0.43}                                    & 0.26                                            & 0.19          & 0.15                                             & \textbf{0.25}                                    & 0.19                                            & 0.19          & 0.17                                             & \textbf{0.31}                                    & 0.21                                            & 0.19          & {\color[HTML]{000000} 0.29}                                             & {\color[HTML]{000000} 0.67}                                             & 0.41                                            & 0.41          & 0.27                                             & 0.44                                             & 0.34                                            & 0.48          & 0.28                                             & 0.52                                             & 0.36                                            & 0.45          \\
Tight grid (improved) & 0.32                                             & 0.39                                             & 0.35                                            & \textbf{0.18} & 0.27                                             & 0.22                                             & 0.24                                            & 0.18          & 0.29                                             & 0.28                                             & 0.28                                            & 0.18          & {\color[HTML]{000000} 0.58}                                             & {\color[HTML]{000000} 0.71}                                             & 0.64                                            & 0.41          & 0.57                                             & 0.47                                             & 0.52                                            & 0.46          & 0.57                                             & 0.55                                             & 0.56                                            & 0.44          \\
Refined grid          & 0.31                                             & 0.36                                             & 0.33                                            & \textbf{0.18} & 0.23                                             & 0.18                                             & 0.20                                            & 0.19          & 0.26                                             & 0.24                                             & 0.25                                            & 0.18          & {\color[HTML]{000000} 0.65}                                             & {\color[HTML]{000000} \textbf{0.76}}                                    & \textbf{0.70}                                   & 0.46          & 0.68                                             & \textbf{0.53}                                    & \textbf{0.59}                                   & 0.51          & 0.67                                             & \textbf{0.60}                                    & \textbf{0.63}                                   & 0.49          \\
Heat-map              & \textbf{0.50}                                    & 0.42                                             & \textbf{0.46}                                   & \textbf{0.18} & \textbf{0.46}                                    & 0.24                                             & \textbf{0.31}                                   & \textbf{0.17} & \textbf{0.48}                                    & 0.30                                             & \textbf{0.37}                                   & \textbf{0.17} & {\color[HTML]{000000} \textbf{0.76}}                                    & {\color[HTML]{000000} 0.64}                                             & \textbf{0.70}                                   & \textbf{0.35} & \textbf{0.77}                                    & 0.40                                             & 0.52                                            & \textbf{0.38} & \textbf{0.77}                                    & 0.48                                             & 0.59                                            & \textbf{0.37} \\ \hline
\end{tabular}
\end{center}
\normalsize
\caption{Output representations results on real test set}
\label{tab:resrepreal}
\end{table*}



==> tables/resrepsynth.tex <==
\begin{table*}[bt]
\footnotesize\addtolength{\tabcolsep}{-5pt}
\begin{center}
\begin{tabular}{|
>{\columncolor[HTML]{FFFFFF}}c |
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c |
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c |
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c |
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c |
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c |
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c |}
\hline
Resolution            & \multicolumn{12}{c|}{\cellcolor[HTML]{FFFFFF}0.3 m}                                                                                                                                                                                                                                                                                                                                                                                                                                                                   & \multicolumn{12}{c|}{\cellcolor[HTML]{FFFFFF}1 m}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                   \\ \hline
Sources               & \multicolumn{4}{c|}{\cellcolor[HTML]{FFFFFF}1}                                                                                                                        & \multicolumn{4}{c|}{\cellcolor[HTML]{FFFFFF}2}                                                                                                                        & \multicolumn{4}{c|}{\cellcolor[HTML]{FFFFFF}Overall}                                                                                                                  & \multicolumn{4}{c|}{\cellcolor[HTML]{FFFFFF}1}                                                                                                                                                                      & \multicolumn{4}{c|}{\cellcolor[HTML]{FFFFFF}2}                                                                                                                        & \multicolumn{4}{c|}{\cellcolor[HTML]{FFFFFF}Overall}                                                                                                                  \\ \hline
Metrics               & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Pre} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Rec} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}F1} & RMSE          & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Pre} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Rec} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}F1} & RMSE          & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Pre} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Rec} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}F1} & RMSE          & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}{\color[HTML]{000000} Pre}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}{\color[HTML]{000000} Rec}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}F1} & RMSE          & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Pre} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Rec} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}F1} & RMSE          & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Pre} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Rec} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}F1} & RMSE          \\ \hline
Tight grid (naive)    & 0.46                                             & \textbf{1.00}                                    & 0.63                                            & 0.12          & 0.35                                             & 0.85                                             & 0.50                                            & 0.15          & 0.39                                             & 0.90                                             & 0.54                                            & 0.14          & {\color[HTML]{000000} 0.46}                                             & {\color[HTML]{000000} \textbf{1.00}}                                    & 0.63                                            & 0.13          & 0.38                                             & 0.91                                             & 0.54                                            & 0.24          & 0.40                                             & 0.94                                             & 0.57                                            & 0.21          \\
Tight grid (improved) & 0.99                                             & \textbf{1.00}                                    & 0.99                                            & 0.09          & 0.83                                             & 0.84                                             & 0.83                                            & 0.12          & 0.88                                             & 0.89                                             & 0.89                                            & 0.11          & {\color[HTML]{000000} 0.99}                                             & {\color[HTML]{000000} \textbf{1.00}}                                    & \textbf{1.00}                                   & 0.09          & 0.92                                             & \textbf{0.93}                                    & 0.92                                            & 0.21          & 0.94                                             & \textbf{0.95}                                    & 0.95                                            & 0.18          \\
Refined grid          & \textbf{1.00}                                    & \textbf{1.00}                                    & \textbf{1.00}                                   & \textbf{0.06} & 0.88                                             & 0.83                                             & 0.86                                            & 0.12          & 0.93                                             & 0.89                                             & 0.91                                            & 0.10          & {\color[HTML]{000000} \textbf{1.00}}                                    & {\color[HTML]{000000} \textbf{1.00}}                                    & \textbf{1.00}                                   & \textbf{0.06} & 0.98                                             & 0.92                                             & \textbf{0.95}                                   & 0.19          & 0.98                                             & 0.94                                             & 0.96                                            & 0.16          \\
Heat-map              & \textbf{1.00}                                    & \textbf{1.00}                                    & \textbf{1.00}                                   & \textbf{0.06} & \textbf{0.93}                                    & \textbf{0.86}                                    & \textbf{0.89}                                   & \textbf{0.10} & \textbf{0.95}                                    & \textbf{0.91}                                    & \textbf{0.93}                                   & \textbf{0.09} & {\color[HTML]{000000} \textbf{1.00}}                                    & {\color[HTML]{000000} \textbf{1.00}}                                    & \textbf{1.00}                                   & \textbf{0.06} & \textbf{0.99}                                    & 0.92                                             & \textbf{0.95}                                   & \textbf{0.16} & \textbf{0.99}                                    & \textbf{0.95}                                    & \textbf{0.97}                                   & \textbf{0.13} \\ \hline
\end{tabular}
\end{center}
\normalsize
\caption{Output representations results on synthetic test set}
\label{tab:resrepsynth}
\end{table*}



